Toward Sequentializing Overparallelized Protocol Code

In our ongoing work, we use constraint automata to compile protocol specifications expressed as Reo connectors into efficient executable code, e.g., in C. We have by now studied this automata based compilation approach rather well, and have devised effective solutions to some of its problems. Because our approach is based on constraint automata, the approach, its problems, and our solutions are in fact useful and relevant well beyond the specific case of compiling Reo. In this short paper, we identify and analyze two such rather unexpected problems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{I. Lanese, A. Lluch Lafuente, A. Sokolova, H. T. Vieira (Eds.):\\
7th Interaction and Concurrency Experience (ICE 2014)\\
EPTCS 166, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.166.5}{10.4204/EPTCS.166.5}}
\pdfoutput=1

